Differentiable Rendering of Neural SDFs through Reparameterization

We present a method to automatically compute correct gradients with respect to geometric scene parameters in neural SDF renderers. Recent physically-based differentiable rendering techniques for meshes have used edge-sampling to handle discontinuities, particularly at object silhouettes, but SDFs do not have a simple parametric form amenable to sampling. Instead, our approach builds on area-sampling techniques and develops a continuous warping function for SDFs to account for these discontinuities. Our method leverages the distance to surface encoded in an SDF and uses quadrature on sphere tracer points to compute this warping function. We further show that this can be done by subsampling the points to make the method tractable for neural SDFs. Our differentiable renderer can be used to optimize neural shapes from multi-view images and produces comparable 3D reconstructions to recent SDF-based inverse rendering methods, without the need for 2D segmentation masks to guide the geometry optimization and no volumetric approximations to the geometry.

==> Makefile <==
R            = main
PACKAGE      = acmart
FIG          = ""
OUTDIR      := output
BUILDIR     := build

PDFFILE := $(OUTDIR)/$(R).pdf

# Final output
pdf: $(PDFFILE)

%.cls:   %.ins %.dtx  
	pdflatex $<

$(PDFFILE): directories $(R).tex sections/*.tex
	./latexrun $(R) -Wall -o $(PDFFILE)

quick:
	pdflatex -draftmode -output-directory=$(BUILDIR) $(R)

directories: 
	mkdir -p $(OUTDIR)
	mkdir -p $(BUILDIR)

clean:
	rm -rf $(BUILDIR) $(OUTDIR) ./latex.out

checksumed:
	mkdir $@

checksum: output/main.pdf checksumed
	timestamp=`date +%s`; cp $< checksumed/teg_$$timestamp.pdf; \
			  md5sum checksumed/teg_$$timestamp.pdf >> checksumed/list.txt;
	tail -n 1 checksumed/list.txt


==> background.bak.tex <==
\section{Background}

\subsection{Discontinuities in Signed Distance Field Rendering}
% Start with 2020-paper

\MG{We should start by introducing differentiable rendering, model parameters and why you need gradients here.}
%
Unlike the neural networks that recent automatic differentiation frameworks were designed for, a rendering pipeline typically exhibits many discontinuities, silhouettes and occlusion chief among them.
%
These discontinuities make correct automatic differentiation of rendering pipelines difficult.
% These discontinuities can arise from various sources, , and they make the rendering function discontinuous. 
%
In this paper, we focus on occlusion discontinuities (or silhouettes) by assuming a differentiable shading model.

%
\input{figures/point_discontinuities}
%
Let $\mathbf{F}(u)$ denote our rendering function, where $u\in\mathbb{R}^2$ is a point on the image plane.
%
In Fig. \ref{fig:point-discontinuities}, we show how a \textit{silhouette} discontinuity makes the rendering function $\mathbf{F}(u)$ non-differentiable at points along the occlusion boundary.
%
In other words, automatic differentiation fails because there exist points $u_{\text{sil}} \in \mathcal{U}_{\text{sil}} \subset \mathcal{U}$ where the derivative of $\mathbf{F}$ w.r.t model parameters $\boldsymbol{\theta}$ does not exist (i.e. $\partial_{\boldsymbol{\theta}}\mathbf{F}(u_{\text{sil}}) \to \pm \infty$)

\MG{a bit vague. what do you mean by 'reasonable'?}
\Sai{I don't want to say 'correct' since a lot of methods use approximations. Is there a better word we ca use here?}
For inverse rendering however, we still need to be able to obtain reasonable gradients inspite of this non-differentiability.
%
There are quite a few different ways in which existing works handle this problem.

\MG{I think most of this paragraph belongs to related work.}
%
For instance, recent approaches in Neural Rendering, such as VolSDF~\cite{} and UNISURF~\cite{} treat the geometry as a volumetric cloud of \textit{occupancy}, in order to remove discontinuities from the rendering model. 
%
In doing so, however, these methods fundamentally \textit{alter} the rendering function (and/or the geometry model). \MG{we should explain why this is undesirable, possibly with some concrete practical issue: bias, less general rendering function that doesn't generalize (next sentence), etc.}
%
These alterations often make the rendering function less general: for example, extending the volumetric shading model in UNISURF and VolSDF to handle global illumination or recover surface reflectance parameters is not trivial.
%
On the other hand, \citet{Yariv:2020:IDR} retain the original SDF rendering model \MG{original from where?} and use the implicit function theorem to compute the correct derivative of intersection points along the ray.
%
However, they account for discontinuities by imposing a secondary loss computed by comparing externally provided segmentation masks with a volumetric occupancy renderer. \MG{say why this is undesirable}


\MG{This would work as intro:}
We ask the question: can we correctly differentiate an SDF renderer without using volumetric approximations for the geometry and the SDF, or information other than RGB images and camera angles (i.e. masks, depth etc.)?

We look to physically-based differentiable rendering for an answer. One key observation made by these approaches is that each pixel (say $\{i, j\}$) is a small integral $\int_{\mathcal{U}_{\text{i,j}}}\mathbf{F}$. \MG{introducing the pixel integral here is a bit odd.}

In this context, there are two broad approaches: \textit{boundary-sampling} and \textit{reparameterization} (sometimes referred to as \textit{area-sampling}).
%
Boundary-sampling methods like \cite{Li:2018:DMC} and \cite{Zhang:2020:PSDR} show, through the Reynolds transport theorem, that the problem of differentiating integrals can be solved by explicitly sampling along the discontinuities in the integration domain.
%
However, both proposed algorithms assume triangle mesh geometry, since they require explicitly enumerating and finding edges that form the silhouette. 
%
These methods don't easily extend to implicitly defined surfaces such as SDFs, because unlike line segments, the silhouette of an SDF has no explicit parametric form that can be used to form samples on it.

Instead we turn to the reparameterization approaches (\cite{Loubet:2019:RDI}, \cite{Bangaru:2020:WAS}) which do not require explicit sampling along discontinuities.


%\begin{enumerate}
%    \item Differentiable rendering is tricky because of discontinuities. The usual approach of running auto-diff on a rendering pipeline doesnt work because each pixel is a discretized version of a small integral over the boundary of the pixel. So how do we handle this?
%    \item If the geometric model in the rendering pipeline is a tri-mesh: Li et al 2019, Zhang et al 2020, 2021 can be used to handle discontinuities through edge/tangent-segment sampling.
%    \item What about a more general rendering pipeline? Recent work (IDR, UNISURF, NeuS, etc..) have used implicit surfaces on real datasets to great effect. Discontinuities are a problem here too, but existing work tends to use various approximations that necessitate either a mask or a volumetric BRDF model. 
%    \item Can we avoid these requirements and still correctly differentiate the pipeline? Unfortunately, tri-mesh based appraoches don't work here since the discontinuities are implicit and not explicit. (cite Fujun's new paper here)
%    \item How can we still correctly differentiate the resulting pipeline? Reparameterization
%\end{enumerate}

\subsection{Reparameterizing Integrals}

\MG{section contains a lot of historical notes that might work better in 'related'}

Reparameterization consists in transforming an integral $\int_{u} f(\mathbf{u}) \mathrm{d}u$,
by changing the variable of integration $u$ using a \emph{diffeomorphic} mapping $\phi$, to obtain an
equivalent integral:
%
\begin{equation}
   \int^{b}_{a}f(\mathbf{u}) \cdot d\mathbf{u} = \int^{\phi^{-1}(b)}_{\phi^{-1}(a)}f(\mathbf{u}') \cdot \left|\partial_{\mathbf{u}}\phi(\mathbf{u})\right|^{-1} \cdot \mathrm{d}\mathbf{u}^{\prime}.
\end{equation}
%
% Note that for the above equality to hold, $\phi(.)$ must be both differentiable and invertible (i.e. a \textit{diffeomorphism}).

The exact form of $\phi$ depends on the goal of this reparameterization --- most often performance.
%
In path-space rendering and variational Bayesian methods for instance, reparameterization is used to
make an integral easier to sample.

\MG{this is related work. I wonder if this paper would not benefit from having the ''background'' + first notations as part of the intro, this would make it easier to discuss the various differences in ''related''.}
Recent differentiable rendering work, however, have a completely different goal: to \textit{inject} a desired derivative into the integral. \cite{Zhang:2020:PSDR}, \cite{Loubet:2019:RDI} and later \cite{Bangaru:2020:WAS} all achieve this through the \textit{infinitesimal} reparameterization $\phi(u) = u + \mathcal{V}(u;\theta)(\theta - \theta_0)$, which effectively inserts a derivative $\partial_{\theta}u^{\prime} = \mathcal{V}(u;\theta)$ without changing the primal value (i.e. $u^{\prime} = u$)

\cite{Bangaru:2020:WAS} refer to the quantity $\mathcal{V}(u;\theta)$ as the warp function, and we will adopt that terminology for this work. \MG{I'd suggest $\mathcal{W}$ for the warp}.
%
For simplicity, we present our derivation assuming $u$ and $\theta$ are scalars (i.e., a 1D pixel with a single parameter).
It naturally extends to higher dimensions: for $\mathbf{u}\in\mathbb{R}^M$ and $\boldsymbol{\theta}\in\mathbb{R}^N$, $\mathcal{V}(\mathbf{u};\boldsymbol{\theta})$ is an $M\times N$ tensor.

\subsubsection{Boundary-aware Warping}\label{sec:boundary-aware-warp}
%
\cite{Loubet:2019:RDI} and \cite{Bangaru:2020:WAS} together use the divergence theorem to show that the gradient contribution from the difficult-to-sample boundary $\mathcal{U}_{\text{sil}}$ can be moved into the easy-to-sample interior $\mathcal{U}$ by finding a suitable warp function $\mathcal{V}(u;\theta)$, and injecting it into the integral through a reparameterization.

How do we tell if a warp function is suitable?
%
\cite{Bangaru:2020:WAS} derive two conditions for this to work: $\mathcal{V}(u;\theta)$ must be (i) continuous for all $u \in \mathcal{U}$, and (ii) it must match the derivative of the discontinuity points when the coordinate $u$ approaches the discontinuity.
%
That is, $\lim_{u \to \mathcal{U}_{\theta{sil}}}\mathcal{V}(u_{\theta{sil}}) = \partial_{\theta}u_{\text{sil}(\theta)}$

In the next section, we (i) form the derivative equation of discontinuity points $\partial_{\theta} u_{\text{sil}}(\theta)$ for a signed distance field renderer, then (ii) propose a warp function $\mathcal{V}^{\text{int}}$ as a weighted integral along the ray, and finally (iii) show an asymptotically consistent approximation $\mathcal{V}^{\text{q}}$ through a quadrature on the intermediate sphere tracer points.



%\cite{Loubet:2019:RDI} was the first paper to propose an alternative to boundary-sampling, choosing to counter-act the effect of parametric discontinuities, by making a suitable parametric transformation that was computed on a per-ray basis through an approximate heuristic. The resulting renderer can then be differentiated using auto-diff frameworks, since the transformation 'removes' the discontinuities (in the infinitesimal neighbourhood of $\boldsymbol{\theta}=\boldsymbol{\theta}_0$). \cite{Bangaru:2020:WAS} refined this approach by showing that the heuristic can be replaced by harmonic convolution in order to account for all of the integral's discontinuities in an unbiased manner. 

While the exact transformation $\phi$ proposed by both \cite{Loubet:2019:RDI} and \cite{Bangaru:2020:WAS} is specific to triangle meshes, the general principle can be applied to any integral over a discontinuous quantity:
For a given instance of parameters $\boldsymbol{\theta} = \boldsymbol{\theta}_0$, the boundary-aware reparameterization is generally of the form $\phi(\mathbf{u}) = \mathbf{u} + \mathcal{V}(\mathbf{u};\boldsymbol{\theta}_0)^T\cdot(\boldsymbol{\theta} - \boldsymbol{\theta}_0)$, where $\mathbf{u}$ is the variable of integration.
Additionally, \cite{Bangaru:2020:WAS} also lays out two requirements for the warp field $\mathcal{V}$ to be 'correct',
(TODO: Add an illustration here showing before and after reparameterization samples to demonstrate continuity and boundary consistency)

Our goal in this work is to show a suitable $\mathcal{V}(\mathbf{u};\boldsymbol{\theta}_0)$

%(TODO: where do we stop the background and start explaining our method?)



%\cite{Bangaru:2020:WAS} also lay out the requirements for a substitution
%Effectively, boundary-aware reparameterization


%They achieve this through a carefully-selected \textit{infinitesimal} transformation $\phi(\mathbf{u}) = R(\mathbf{u};\theta)$
%Often, integrals are reparameterized to modify the characteristics of the inner integrand without changing the integrated value.
%Cite Loubet 2019 \& 2021 and Bangaru 2020 for the boundary-aware reparameterization method. 

%\begin{enumerate}
%    \item Express that reparameterization in Bangaru 2020 is a form of boundary-aware warping that can be used to re-write samples
%    such that the pipeline is no longer discontinuous.
%    \item Requires find a warp function $V(u;\theta_0)$ that is consistent at discontinuities (note that it is not unique, and the variance of the resulting estimator depends on the exact structure of $V(u;\theta_0)$). Bangaru 2020 and Loubet 2019, 2021 use an inner convolution that works for triangle meshes.
%    \item What about implicit surfaces such as SDFs? Can we be more explicit here?
%\end{enumerate}


==> figures/notations.tex <==
\begin{table}[t]\caption{Notation}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{r c p{5cm} }
\toprule
$u \vcentcolon \mathtt{R}^2$ & $\triangleq$ & Image space coordinate \\
$\mathbf{x} \vcentcolon \mathtt{R}^3$ & $\triangleq$ & 3D points \\
$\mathcal{U} \subseteq \mathtt{R}^2$ & $\triangleq$ & Image/pixel space (set of all $u$ in a pixel) \\
$\mathcal{X} \subseteq \mathtt{R}^3$ & $\triangleq$ & 3D Euclidean space (set of all $X$) \\
$\mathcal{U}_{\text{sil}} \subseteq \mathtt{R}^2$ & $\triangleq$ & Set of silhouette points in $\mathcal{U}$ \\
$\mathcal{X}_{\text{sil}} \subseteq \mathtt{R}^3$ & $\triangleq$ & Set of silhouette points in $\mathcal{X}$ corresponding to $\mathcal{U}_{\text{sil}}$ \\
$\boldsymbol{\theta} \vcentcolon \mathtt{R}^{N} $ & $\triangleq$ & N-D geometry parameters \\
$f(\mathbf{x}; \boldsymbol{\theta}) \vcentcolon \mathtt{R}^{3\times N} \to \mathtt{R} $ & $\triangleq$ & Signed distance function \\
$F(u; \boldsymbol{\theta}) \vcentcolon \mathtt{R}^{2\times N} \to \mathtt{R} $ & $\triangleq$ & Radiance along the ray from $u$\\
$\partial_{\boldsymbol{\theta}}f \vcentcolon \mathtt{R}^{3\times N} \to \mathtt{R}^N  $ & $\triangleq$ & Partial derivative of $f$ w.r.t geometry parameters\\
$\partial_{\mathbf{x}}f \vcentcolon \mathtt{R}^{3\times N} \to \mathtt{R}^3  $ & $\triangleq$ & Partial derivative of $f$ w.r.t spatial dimension. Normal direction of the SDF.\\
$G(\mathbf{x}; \theta)\vcentcolon \mathtt{R}^{3\times N} \to \mathtt{R}^{N\times 3}  $ & $\triangleq$ & Geometric derivative w.r.t each  $\boldsymbol{\theta}$\\
$\partial_{\mathbf{x}}u \vcentcolon \mathtt{R}^{3} \to \mathtt{R}^{3\times 2}  $ & $\triangleq$ & Jacobian of projection $\mathcal{X} \to \mathcal{U}$ $\boldsymbol{\theta}$\\
$\mathcal{V}(u; \theta)\vcentcolon \mathtt{R}^{2\times N} \to \mathtt{R}^{N\times 2}  $ & $\triangleq$ & Warp function on pixel coordinates $u$\\
\bottomrule
\end{tabular}%
}
\label{tab:notation}
\end{table}

==> figures/point_discontinuities.tex <==

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/nondiff_rendering_function}
    \caption{\label{fig:point-discontinuities}
    }
\end{figure}

==> figures/weights_abl.tex <==
\begin{figure}[!tbh]
\centering
\setlength{\tabcolsep}{1pt}
\begin{tabular}{ccc}
\includegraphics[width=0.2\linewidth]{figs/holder.png} &
\includegraphics[width=0.2\linewidth]{figs/holder.png} &
\includegraphics[width=0.2\linewidth]{figs/holder.png} \\
ground truth & $\gamma=0.5$ & $\gamma=2.0$
\end{tabular}
\caption{\textsc{Ablation gamma.} }
\label{fig:ablation-wts}
\end{figure}

==> sections/_background_backup.tex <==
% \cite{Zhang:2020:PSDR}, \cite{Loubet:2019:RDI} and later \cite{Bangaru:2020:WAS} all achieve this through the \textit{infinitesimal} reparameterization $\phi(u) = u + \mathcal{V}(u;\theta)(\theta - \theta_0)$, which effectively inserts a derivative $\partial_{\theta}u^{\prime} = \mathcal{V}(u;\theta)$ without changing the primal value (i.e. $u^{\prime} = u$)
% \subsection{Reparameterizing Integrals}

% \MG{section contains a lot of historical notes that might work better in 'related'}
% \KS{I agree with Michael. Why not just start with the warp-based integral. i.e., Eqn. 5 in Bangaru? Otherwise this section reads like the related work/background section for Bangaru.}

% Reparameterization consists in transforming an integral $\int_{u} f(\mathbf{u}) \mathrm{d}u$,
% by changing the variable of integration $u$ using a \emph{diffeomorphic} mapping $\phi$, to obtain an
% equivalent integral:
% %
% \begin{equation}
%    \int^{b}_{a}F(\mathbf{u}) \cdot d\mathbf{u} = \int^{\phi^{-1}(b)}_{\phi^{-1}(a)}F(\mathbf{u}') \cdot \left|\partial_{\mathbf{u}}\phi(\mathbf{u})\right|^{-1} \cdot \mathrm{d}\mathbf{u}^{\prime}.
% \end{equation}

% The exact form of $\phi$ depends on the goal of this reparameterization --- most often performance.
% %
% In path-space rendering and variational Bayesian methods for instance, reparameterization is used to
% make an integral easier to sample.

% \MG{this is related work. I wonder if this paper would not benefit from having the ''background'' + first notations as part of the intro, this would make it easier to discuss the various differences in ''related''.}
% \KS{I agree. Also the previous equation uses a generic integral. Here you are suddenly introducing the notion of scene parameters $\theta$, a pixel $u$, etc. I would recommend you start from Eqn. 5 in Bangaru and explain all the parts and then proceed.} 

% Related \KS{One of our main goal in this work is to derive a suitable form for the warp function for neural SDFs.
%$\mathcal{V}(\mathbf{u};\boldsymbol{\theta}_0)$}

%\KS{Drop this para, it's a repeat of the previous.}
%While the exact transformation $\phi$ proposed by both \cite{Loubet:2019:RDI} and \cite{Bangaru:2020:WAS} is specific to triangle meshes, the general principle can be applied to any integral over a discontinuous quantity:
%For a given instance of parameters $\boldsymbol{\theta} = \boldsymbol{\theta}_0$, the boundary-aware reparameterization is generally of the form $\phi(\mathbf{u}) = \mathbf{u} + \mathcal{V}(\mathbf{u};\boldsymbol{\theta}_0)^T\cdot(\boldsymbol{\theta} - \boldsymbol{\theta}_0)$, where $\mathbf{u}$ is the variable of integration.
%Additionally, \cite{Bangaru:2020:WAS} also lays out two requirements for the warp field $\mathcal{V}$ to be 'correct',
%(TODO: Add an illustration here showing before and after reparameterization samples to demonstrate continuity and boundary consistency).
%\subsection{The Rendering Pipeline}
%Explain the components of the pipeline. The specifics of each component are not very important. (TODO: Illustration here to show the image pixel space, camera transform, the sphere tracer points and then finally the shader)
%In a abstract sense, the color value of each pixel can be represented as an integral over the values of each point $u$ in the set $\mathcal{U}_{i,j}$ that cover the pixel $i, j$ in image space.
%The value of each point $u$ is the radiance computed by the shader $S$ for the intersection point computed by our solver $T$ for the ray computed by our camera model $C$. 
%$I = \int_{\mathcal{U}_{i,j}} (S \circ T \circ C)(\mathbf{u};\boldsymbol{\theta})$(Note that in practice each module has additional inputs that we're ignoring here for clarity)
%TODO: Quickly explain that $S$ is IDR's radiance network (NeRF-like but evaluated at surface points only), $T$ is a standard sphere tracing algorithm, and $C$ is the perspective camera transform with a Box or Gaussian filter.
%Now that we have our primal renderer, can we differentiate it for use in inverse rendering applications? Unfortunately, like most tri-mesh renderers, implicit surface renderers also contain discontinuities, with the added caveat that, in general, it's impossible to represent the silhouettes in an explicit parameteric form. 
%(mention here that the discontinuities in pixel filters are not an issue since it's trivial to obtain their parametric form). 

%This means that one of two broad approaches to unbiased differentiable rendering: edge/boundary sampling doesn't apply here (TODO: mention marching cubes + existing methods?). However, the reparameterization method does not require sampling points on the boundary.

%As mentioned in the background section, reparameterization substitutes the image space coordinate $u$ in the integral $I$ with a new $u^{\prime} = u + \mathcal{V}(\mathbf{u}; \boldsymbol{\theta}_0)^T (\boldsymbol{\theta} - \boldsymbol{\theta}_0)$ such that the resulting integral $I'$ (i) has the same primal value at $\boldsymbol{\theta}=\boldsymbol{\theta}_0$ by construction, and (ii) is now fully differentiable because the integrand $S \circ T \circ C$ is continuous.

%Our goal then is to find a describe a warp field that works for implicit surfaces and show a way to compute this using information already available in the primal rendering pass. We show that unlike existing reparamterization methods, we do not need expensive convolutional rays to produce the correct warp.

%\begin{enumerate}
%    \item Similar to prior work (Bangaru, Loubet), it is insufficient to use only the intersection point to compute the warp field. Intuitively, this is because the intersection point does not have \textit{any} information about surfaces that are \textit{close} to the ray. Prior work solves this by launching additional auxiliary rays to 'map' the surrounding area.
%    \item We don't need to do this, since implicit representations already contain this information!
%    \item How do we take advantage of this? In this paper we design a warp field for implicit surfaces which, when used to reparameterize the renderer produces unbiased derivatives inexpensively by repurposing the points of a sphere tracer.
%\end{enumerate}

%$w(\mathbf{d} + t\cdot\mathbf{o}, \vec{\mathbf{d}})/\int^{t^{\prime}_0}_{t^{\prime}=0} w(\mathbf{d} + t^{\prime}\cdot\mathbf{o}, \vec{\mathbf{d}}) = 1$ where $\vec{\mathbf{o}}(u) + t\cdot\vec{\mathbf{d}}(u)$

% |_{\mathbf{x}=\vec{\mathbf{o}}(u) + t\cdot\vec{\mathbf{d}}(u)}
% 




%Intuitively, this quantity represents how a discontinuity position changes w.r.t.\ a geometry parameter $\theta$. 
%
%Since $u_{\text{sil}}$ is not a readily available quantity, its derivative expression is not trivial to determine. 
%
%Fortunately, this problem has been tackled by existing differentiable rendering work (both explicit and implicit differentiation).
%
%Li et al. \shortcite{Li:2018:DMC}, Bangaru et al. \shortcite{Bangaru:2020:WAS} and Loubet et al. \shortcite{Loubet:2019:RDI}, all show how to compute this quantity for a triangle mesh by computing the derivative of the intersection point $\mathbf{x}$ w.r.t $\boldsymbol{\theta}$ independent of the ray, and projecting that derivative using the Jacobian of $\mathbf{x}$ w.r.t $u$. 
%
%The method used by existing approaches to compute $\partial_{\theta}\mathbf{x}$ assumes a triangle mesh, often computed by fixing barycentric coordinates. \KS{This whole para is previous work. I suggest cutting it down and moving the important parts to the ``Background'' subsection.}

% TODO: Cite material form
%This definition does not directly transfer to implicit surfaces, since surface points do not have a unique identity (the same reason why it is difficult to uv-map an implicit surface).
%

%Fig. \ref{fig:du-dtheta} shows how we can Some definitions: (TODO: Explain through illustrations)
%Let's define $\mathcal{U}_{\text{sil}}$ to be the set of points in \textbf{pixel space} $\mathcal{U}_{i,j}$ that are discontinuous (i.e. silhouettes), and $\mathcal{X}_{\text{sil}}$ be the set of \textbf{3D points} on the surface that make up the silhouette. For this discussion, these sets are defined for a specific camera position, although in practice our formulation works for any arbitrary origin.
%In \cite{Bangaru:2020:WAS}, the authors lay out two requirements on the warp function for the result to be unbiased: (i) \textit{Continuitity} and (ii) \textit{Boundary Consistency}. Intuitively, boundary consistency says that, at a discontinuity point $\mathbf{u}_{\text{sil}}$, $\mathcal{V}_{\theta}$ has the same value as the derivative $\mathbf{u}_{\text{sil}}$ w.r.t parameters $\boldsymbol{\theta}$. In \cite{Bangaru:2020:WAS}, the authors define this for triangle meshes through the \textit{material form} (formally defined in \cite{Zhang:2020:PSDR}) by 'attaching' the point to the surface as shown in Fig. 5a of \shortcite{Bangaru:2020:WAS}.

%This definition does not directly transfer to implicit surfaces, since surface points do not have a unique identity (the same reason why it is difficult to uv-map an implicit surface). Fortunately, we can define a consistent material form for implicit surfaces through the implicit function theorem (cite..). For an implicit function $f(\mathbf{x}; \boldsymbol{\theta})$, the derivative of a 3D point $\mathbf{x}$ on the surface w.r.t parameters $\boldsymbol{\theta}$ is given by 
%$$ \partial_{\boldsymbol{\theta}} \mathbf{x} = \frac{\partial_{\boldsymbol{\theta}} f \partial_{\mathbf{x}} f^T}{\|\partial_{\mathbf{x}} f\|^2} $$
%To get the derivative in pixel coordinates $\mathbf{u}$, we will have to transform this derivative by the Jacobian $(\partial_\mathbf{u}x)^{-1}$


==> sections/background.tex <==
\section{Background}


